Unprecedented Code Change Automation: The Fusion of LLMs and Transformation by Example

Software developers often repeat code changes, known as "code change patterns" (CPATs), within and across projects. Automating these CPATs accelerates development, but current Transformation by Example (TBE) techniques are limited by the input examples' quality and quantity, missing variations with different syntax or flow yet semantically similar. Large Language Models (LLMs), trained on vast code datasets, can overcome these limitations by generating semantically equivalent, unseen CPAT variants, enhancing TBE effectiveness. We identified best practices for using LLMs to generate code variants meeting criteria of correctness, usefulness, and applicability. Implementing these in PyCraft, combining static and dynamic analysis with LLMs, we achieved an F-measure of 96.6% in identifying correct variants, expanding inputs by 58x on average, and automating changes to increase target codes by up to 39x. Patches from PyCraft were submitted to projects like microsoft/DeepSpeed and IBM/inFairness, with an 83% acceptance rate, validating our approach's usefulness.

==> Background.tex <==
\section{Background}
In this section, we provide a brief overview of the background knowledge relevant to this paper, including Transformation By Example (TBE) and Large Language Models (LLMs).


In practice, a prompt can incorporate anything that can be captured in textual format. In particular, multi-modal prompts are those that incorporate different modalities of inputs, such as natural language, code, and data.
% http://iri-pycpt.github.io


We use the following terminologies throughout the paper. 
\begin{enumerate}[label=(\roman*),wide, labelwidth=!,labelindent=0pt]
\item Transformation By Example (TBE): is an approach used to automatically generate code transformations based on a given set of example transformations.
It involves specifying the desired input-output behavior and allowing the system to infer the underlying transformation rules. 
TBE has been widely studied and applied in various software engineering tasks, such as code refactoring and synthesis.

\item Large Language Models (LLMs): are powerful machine learning models that have been trained on vast amounts of text data, including source code from software repositories. These models, such as GPT-3, are capable of generating coherent and contextually relevant code snippets based on given prompts. LLMs have demonstrated their potential in various software engineering tasks, including code completion, code summarization, and natural language code understanding.


\item CPAT: We mine CPATs using \textit{R-CPATMiner}~\cite{rcaptminer2022ICSE}. A CPAT contains three or more instances of code changes that have been performed in the commit history of Python projects. A code change instance contain deleted code known as LHS (red colored code in \Cref{fortonumpy}) and then inserted code known as RHS (green colored code in \Cref{fortonumpy}). 
% \item Unseen variant: The rule synthesizer infers rules using the output of \textit{R-CPATMiner}~\cite{rcaptminer2022ICSE}. Then, these rules can be applied to the target codes in order to perform the same change. 
% Each code change instance includes deleted code, known as LHS (highlighted in red in \Cref{fortonumpy}), and inserted code, known as RHS (highlighted in green in \Cref{fortonumpy}). 

% #todo
% \item Data, Control-flow variants:
% Applying CPATs to the real-world is tricky, often because real code doesn't match the LHS of a transformation rule perfectly. It is common for real code to slightly differ from the LHS in terms of data-flow or control flow. Such variants have the same semantics are the LHS; however, applying the transformation rule to such variants is not a straightforward process. 



% Listing \ref{lst:df_fortonumpy} is an example of a data-flow variant. It is semantically equivalent to Listing \ref{fortonumpy} but has additional variable, modifying the data flow of the code-block.

% Listing \ref{lst:cf_fortonumpy} is an example of a control-flow variant of listing \ref{fortonumpy}. Here, there is a call to a method, to retrieve the iterable contents. Again, it is equivalent to Listing \ref{fortonumpy}.

% \begin{lstlisting}[language=Python, caption=A data-flow variant for Listing \Cref{fortonumpy}\label{lst:df_fortonumpy},style=tablecode]

% result = 0
% for i in sorted(elements):
%     total = result + i
%     result = total
    
% \end{lstlisting}

% \begin{lstlisting}[language=Python, caption=A control-flow variant for Listing \Cref{fortonumpy}\label{lst:cf_fortonumpy},style=tablecode]

% result = 0
% for i in get_elements():
%     result += i
    
% \end{lstlisting}



% \item Large Language Models (LLM):
% LLMs are the new cutting edge natural language processing machines. They are trained on massive amounts of dat
% \item Hallucinations:

% Responses from LLMs are sometimes made up and are not factual; even though they seem to be real. This is a a downside to the creative powers of LLMs. Such behaviour is termed a 'hallucination'. LLMs sometimes hallucinate when asked to provide variants. We observe hallucinations in the form of unreasonable code, which no real developer would write. Listing \ref{lst:hal_fortonumpy} provides an example of Listing \ref{fortonumpy}. There is no reason a developer would sort a listing before summing over its elements. Even though such variants are semantically equivalent to the original, they hamper the quality of our technique. Thus, it is important to weed hallucinations out.

% \begin{lstlisting}[language=Python, caption=A hallucinatory variant for Listing \Cref{fortonumpy}\label{lst:hal_fortonumpy},style=tablecode]

% result = 0
% for i in sorted(elements):
%     result += i
    
% \end{lstlisting}

% \item Chain of Thought Reasoning:

% When asked to perform larger and more complicated tasks, LLMs can sometimes jump to conclusions, leading to erroneous responses. To achieve more accurate responses from LLMs, it helps to list out actionable steps to be taken by the LLM to perform it's task. Providing a Chain of Thought in the prompt is essential for an LLM to accurately reason about complex tasks. 
% We employ this method extensively in our prompts. 

\end{enumerate}


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> RQ3.tex <==


\subsection{RQ3: Best performing parameters generating test cases\label{sec:rq3}}
\tool generates testcases to determine semantically equivalent variants for the original \cpat.
Here, we utilize LLM and then prmpt it multiple times with the same prompt to generate test cases for one \cpat, which allows LLM to generate divers test cases, as
they impact randomness and iterative exploration,






To achieve optimal generation for both test case and variant generation, LLMs requires meticulous fine-tuning of values for the parameters: Temperature ($T$), Iterations for prompt input ($I_p$), and Iterations for fixed-point iterations ($I_f$) (The parameters are detailed in \ref{sec:tuning_parameters}).
To determine optimal values, we adopt an empirical approach.
We first generated an oracle of unseen variants consist with 
9325 unseen variants for 10 \cpats given \Cref{table:cpat}. 
Then, we used both automated and manual steps to group the variants into \textit{Correct variants} (\Cref{def:correctvariant}), \textit{Useful variants} (\Cref{def:usefulvariant}), and \textit{Applicable variants} (\Cref{def:applicablevariant}). We utilized this oracle to investigate primarily two sub-research questions:
\begin{enumerate*}[label=(\roman*)]
\item \textit{What are the optimal parameters for generating test cases?} 

\item \textit{What are the optimal parameters for generating unseen variants?}
\end{enumerate*}
Through the study of these research questions, we determine the best-performing values for $T$, $I_p$, and $I_f$ for generating variants and test cases. This enables \tool to utilize LLMs to their fullest potential.


% parameters based on the oracle to produce efficient test cases (\Cref{sec:gentestcases}) and reduce hallucinations during variant generation (\Cref{sec:genvariants}).



% \begin{figure}[htbp]
%     \includegraphics[width=0.49\textwidth,keepaspectratio]{images/tuning_parameters.pdf}
% \vspace{-4mm}
%     \caption{Schematic diagram of the workflow for generating data to fine-tune LLM parameters}
%     \label{fig:empirical}
% \vspace{-5mm}
% \end{figure}




\subsubsection{\textbf{Creating an oracle:}\label{sec:oracal}}
As shown in \Cref{fig:empirical}, we invoke LLM to generate unseen variants for the 10 CPATs
shown in \Cref{table:cpat}.
Our objective is to generate the full set of unseen variants for each CPAT. 
We generate 10 such sets, and each set is denoted as $V^m$, where $m$ corresponds to the CPAT number ($m \in \{1, 2, \ldots, 10\}$).
To create $V^m$, we prompted LLM with \cpat $m$ for each temperature value in the set $\{0, 0.3, 0.5, 0.7, 0.9, 1.2\}$.
For each temperature value, we performed prompt iterations ($I_p$) up to 15 times, by repeatedly prompting the LLM with the same CPAT.
After completing all 15 prompt iterations, we employed fixed-point iteration, inputting each generated variant back into the LLM. We repeated these steps until no new variants were generated.
Through this process, a total of 9325 distinct variants were generated for all CPATs.







% To generate $V^p$, we prompted LLM for each temperature value, $\{0, 0.3, 0.5, 0.7, 0.9, 1.2\}$ and for each prompt iteration ($I_p$) value within the set $\{1, 2, 3, \ldots, 15\}$ by prompting the same prompt with the identical variant. 
% We also performed fixed-point iterations ($I_f$) by repeatedly providing the generated variant as input to the LLM until no new variant is generated.


\begin{figure}[t]
    \begin{minipage}[b]{0.5\linewidth}
        \centering
\includegraphics[height=2cm,keepaspectratio=true]{images/tuning_parameters.pdf}
         \vspace{-5mm}
    \caption{Schematic diagram of the workflow for generating data to fine-tune LLM parameters}
    \label{fig:empirical}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.38\linewidth}
        \centering
        \includegraphics[width=5cm,keepaspectratio=true]{images/prompt_iteration/line_plot.pdf}
         \vspace{-4mm}
        \caption{Generation of variants (Y-axis) along with prompt iteration (X-axis)}
        \label{fig:promptIteration}
    \end{minipage}
    \vspace{-5mm}
\end{figure}




% As shown in Figure \ref{fig:empirical}, we initially select 10 \cpats, denoted as $C$, from the output of \textit{R-CPATMiner} by running it on \numbProjects open source Python repositories. Subsequently, we invoked LLM to generate unseen variants for the selected \cpats. Our objective is to generate the set of all possible unseen variants for the chosen \cpats, denoted as $V^p$ where $p \in \{1, 2, 3, \ldots, 10\}$.
% To achieve this, we generate variants for each temperature value in the set $\{0, 0.2, \ldots, 1.2\}$ and for each iteration value in the set $\{1, 2, 3, \ldots, 10\}$. Thus, we invoke LLM for each \cpat $c \in C$ and for each combination of temperature $t \in \{0, 0.2, \ldots, 1.2\}$ and iteration $i \in \{1, 2, 3, \ldots, 10\}$, resulting in the generation of total \rqfourUnseenVariants unseen variants, for all $V^p$.

As the next step, two authors of the paper manually wrote unit test cases for the \cpats to evaluate their functionality and consider boundary cases. 
Then, we executed the test cases on the generated unseen variants to classify them as either correct ($V_c^m$) or incorrect ($V_i^m$). 
This classification process resulted in total \rqfourVI incorrect variants ($\sum_{m=1}^{10}$ $V^m_i$) and \rqfourVC correct variants ($\sum_{m=1}^{10}$ $V^m_c$).
% The classification for 10 CPATs is summarized in \Cref{table:cpat}.

To categorize the correct variants ($V^m_c$) into "Usable" (\Cref{def:usefulvariant}), referred to as ($V^m_u$), we utilized the Inter-Rater Reliability (IRR) methodology~\cite{landis1977measurement}. Following best practices and qualitative research guidelines, the authors employed a negotiated agreement technique~\cite{wicks2017coding, campbell2013coding} to achieve consensus.
Two authors of the paper conducted manual analyses on each change pattern to identify the high-level programming tasks associated with them. They reached a consensus to classify a variant as ``usable'' if it represented something a developer would realistically write, and they labeled variants as ``not useful'' if developers would not typically include them in their code.
Then, we conducted the static analysis given in \Cref{sec:applicable} to further identify the ``applicable'' variations ($V^m_a$) from the ``useful'' variants. With this process, we identified a total of \todo{1211} useful variants ($\sum_{m=1}^{10}$ $V^m_u$) and \todo{211} applicable variants ($\sum_{m=1}^{10}$ $V^m_a$).
This data set serves as a resource for fine-tuning variables during the generation of test cases and variants as explained in the following sections.

% Two authors of the paper performed manual analysis on each change pattern to identify the high-level programming tasks associated with them. 
% Independently, the authors carefully examined the unseen variants and assigned them codes of ``\usable" and ``not-useful" based on their assessments. 

% Following best practices and guidelines for qualitative research, the authors utilized a negotiated agreement technique~\cite{wicks2017coding,campbell2013coding} to achieve consensus. 

% To ensure the reliability of the coding process, both authors conducted an initial meeting after coding approximately 25\% of the data, surpassing the suggested minimum size, i.e., 10\% ~\cite{campbell2013coding}. 
% During this meeting, they thoroughly discussed the coding process and resolved any disagreements regarding patterns that did not align with high-level program transformations. After achieving an inter-coder agreement of 80\% (recommended inter-coder agreement level ranges from 70\% to more than 90\% in the literature~\cite{campbell2013coding}), the authors independently completed the coding for the remaining variants. This rigorous approach ensures the reliability and validity of the categorization process and forms a solid foundation for subsequent analysis.
% The analysis result is summarized in the \Cref{table:cpat}.
% The authors identified \rqfourVU \usable useful variants and a subset of \rqfourVA \applicable variants.
% Then, we conducted the static analysis given in \Cref{sec:applicable} to further identify the ``applicable''  variations ($V^m_a$) from the ``useful'' variants.
% With this process we identified total \todo{1211} useful variants
% ($\sum_{m=1}^{10}$ $V^m_u$) and \todo{211} applicable variants ($\sum_{m=1}^{10}$ $V^m_a$).


% This dataset serves as a valuable resource for fine-tuning variables during the generation of test cases and variants as explained in the following sections.

\subsubsection{\textbf{What are the optimal parameters for generating test cases?}\label{sec:gentestcases}}
\tool uses the test cases to determine the semantic equivalence between the generated variants and the original \cpat. 
Therefore, our goal is to identify the most effective combination of values for temperature ($T$) and prompt iterations ($I_p$) for test case generation, aiming to produce high-quality test cases.


\textbf{Dataset and Experimental setup:}
To study the optimal parameters for test case generation, we study the quality of the generated test cases for a range of Temperature (\(T\)) values, from the set \(\{0, 0.2, 0.4, 0.6, 0.8, 1.0, 1.2\}\), and prompt iterations (\(I_p\) = \(\{1,2, \dots, 15\}\)).
% by prompting the same prompt to generate test cases.
We generate a set of test cases using LLM for each \cpat, considering each \((t, i)\) combination where \(t \in T\) and \(i \in I_p\). 
These generated test cases are then subjected to the three-step validation process utilized by \tool.
This process enables us to identify and select the valid test cases, denoted as \(T^m_{(t,i)}\), across diverse \(T\) and \(I_p\) values.
We then study the effectiveness of testcases, by
executing each set of test cases, $T^m_{(t,i)}$, on the oracle $V^m$ (described in \Cref{sec:oracal}) and classified them into correct variants $\overline{V}^m_c$ and incorrect variants $\overline{V}^m_i$, and then compare them to the classified variants \(V^m_i\) and \(V^m_c\) in the oracle.
To evaluate the effectiveness of generated test cases in classifying variants as correct or incorrect, we calculated precision and recall. 
Precision is the percentage of correct variants (\(\overline{V}^m_c \cap V^m_c\)) among the variants classified as correct (\(\overline{V}^m_c\)), while recall is the percentage of correctly identified variants among all actual correct variants in the oracle (\(V^m_c\)).
Then, we compute F-measure using precision and recall values which is the harmonic mean of precision and recall, calculated as \(\frac{2 \cdot (\text{precision} \cdot \text{recall})}{\text{precision} + \text{recall}}\).

% We use the oracle generated in \Cref{sec:oracal}.
% As shown in Figure \ref{fig:testgen}, we generated test cases, known as $T^p_{(t,i)}$, for each CPAT using the LLM, for all combinations of temperature, $t \in \{0, 0.2, \ldots, 1.2\}$ and iterations, $i \in \{1, 2, 3, \ldots, 10\}$, for each CPAT $p \in \{1, 2, 3, \ldots, 10\}$.
% Subsequently, we executed each group of test cases, $T^p_{(t,i)}$, on the oracle $V^p$ generated for each CPAT as described in Section \ref{sec:oracal} and classified them into correct variants $V^p_c$ and incorrect variants $V^p_i$.
% Then we compared each classified variant $V^p_i$ and $V^p_c$ to the classified variants using human-generated tests explained in Section \ref{sec:oracal}.
% We then computed the precision (percentage of correctly classified $V^p_c$ variants), denoted as \text{$P^p$}(t,i),  and recall, denoted as \text{$R^p$}(t,i), (percentage of correctly classified $V^p_c$ variants among all $V^p_c$ in the oracle) to assess effectiveness of LLM generated test cases on classifying the variants into correct and incorrect.



% \begin{figure}[htbp]
%     \includegraphics[width=0.49\textwidth,keepaspectratio]{images/test-case-heatmaps/precision-recall/average.png}
%     % \includegraphics[width=0.49\textwidth,keepaspectratio]{images/test-case-heatmaps/test.pdf}

%     \caption{Precision and Recall for the CPAT in \Cref{fortonumpy}.}
%     \label{fig:test_heatmap}
% \end{figure}


% \begin{figure}[htbp]
%   \begin{minipage}{0.25\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/cross-validation/cross-validation precision.pdf}
%     \caption{Caption for Image 1}
%     \label{fig:image1}
%   \end{minipage}%
%   \begin{minipage}{0.25\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/cross-validation/cross-validation recall.pdf}
%     \caption{Caption for Image 2}
%     \label{fig:image2}
%   \end{minipage}
% \end{figure}



% \begin{figure}[htbp]
% \vspace{-2mm}
% \hspace{-2mm}
% \subfigure[Precision\label{fig:cross_precision}]{
% \includegraphics[width =0.35\textwidth]{images/cross-validation/cross-validation precision.pdf}}\hspace{-1mm}
% \subfigure[Recall\label{fig:cross_recall}]{
% \includegraphics[width =0.35\textwidth]{images/cross-validation/cross-validation recall.pdf}}
% \hspace{-4mm}
% \vspace{-2mm}
% \caption{Cross-validation results for learning optimal $i$ and $t$ values and applying them to other CPATs\label{metrics}}
% \vspace{-3mm}
% \end{figure}

% \begin{figure}[htbp]
%     \includegraphics[width=0.49\textwidth,keepaspectratio]{images/prompt_iteration/line_plot.pdf}

%     \caption{}
%     \label{fig:promptIteration}

% \end{figure}




% To find the optimal values of \(i\) and \(t\) that yield the most effective test cases, achieving the best precision and recall, we utilize the F-measure. The F-measure is the harmonic mean of precision and recall, calculated as \(\frac{2 \cdot (\text{precision} \cdot \text{recall})}{\text{precision} + \text{recall}}\).
% \alpha \cdot P(t, i) + \beta \cdot R(t, i)$, where $\alpha$ and $\beta$ are weight parameters. 
% We choose $\alpha > \beta$ to prioritize precision in classifying correct variants over recall, as correctly detecting the variant is more critical than detecting all correct variants for the tool. 
To identify the most effective combinations of \(i\) and \(t\), we adopt the following approach: For each fixed value of \(i\), we calculate the F-measure for all \(t\) values. 
Then, for each \(i\), we identify the \(t\) value that yields the maximum F-measure, denoted as \(\max_{t \in T} F(t, i)\), along with the corresponding \(t\) value, denoted as \(t_{\text{max}}\). 
To further refine this process, we introduce a convergence criterion. If the difference between the maximum F-measure of the current iteration, \(F(t_{\text{max}}, i)\), and the maximum F-measure from the previous iteration, \(F(t_{\text{max}}, i-1)\), exceeds a threshold \(\delta\), we increment \(i\) by 1 and repeat the procedure. 
This iterative refinement goes until the F-measure no longer improves by more than \(\delta\).
We have chosen \(\delta\) to be 5\% to ensure swift convergence based on the observed data.

% value compared to the previous iteration is greater than or equal to the threshold $\delta$ (i.e., $F(t_{\text{max}}, i) - F(t_{\text{max}}, i-1) \geq \delta$), we update the value of $i = i + 1$). 
% We repeat this until the improvement in $F(t_{\text{max}}, i)$ falls below the threshold $\delta$ or until $i$ reaches the maximum value in $I$. B
% y following this approach, we explore different $t$ values for each fixed $i$ to find the optimal combination of $t$ and $i$ that maximizes the objective function while minimizing the number of iterations.




After selecting a specific $(t, i)$ combination for $V^p$ that effectively generates test cases to classify the variants, we perform 10-fold cross-validation to assess whether this chosen combination learn from one \cpat can be generalized to other CPATs. 
Let $V^m$ be a set of variations generated for a CPAT, where $m \in {1, 2, 3, \ldots, 10}$. 
After obtaining the optimal combination $(t, i)$ for $V^m$, we then apply this learned combination to all the other $V^{m'}$s, where $m' \in {1, 2, 3, \ldots, 10}$ and $m' \neq m$. 
% In other words, we use the same $(t, i)$ values to generate test cases for each $V^{p'}$ in the dataset, 
This allows us to assess how well this combination generalizes to different patterns.


\textbf{Results:}
\Cref{fig:metrics} shows the cross-validation results. 
The x-axis represents the $(t, i)$ configurations that achieved the best precision or recall values for each CPAT index (refer to \Cref{table:cpat} for index to CPAT mapping), while the y-axis represents CPAT index.
The outcomes of k-fold cross-validation involve applying the learned \((t, i)\) values to generate test cases with \tool for other patterns and then calculating their precision and recall values, which are displayed in the respective cells.
% The shaded cells represent the highest achieved precision or recall values for the corresponding $t, i$ values and the respective CPATs on the x-axis.



The analysis consistently shows that $t = 1.2$ yields higher precision and recall performance, indicating that LLM with higher randomness is better suited for test case generation. Additionally, the number of iterations varies between $3$ and $10$ for each CPAT, with higher iterations generally resulting in similar or better precision and recall. However, to strike a balance between effectiveness and efficiency, we choose the value for $i = 5$, which provides superior precision and recall for \cpats. 
The combination of $(t, i)$ strikes a balance between precision, recall, and efficiency, making it the ideal setting for test case generation by \tool with precision and recall rates of \testcaseAvePrecision and \testcaseAveRecall.

% \Cref{fig:cross_precision} and \Cref{fig:cross_recall} provide an overview of the cross-validation process results. The x-axis represents the $(t, i)$ configurations that achieved the best precision or recall values for each CPAT. The y-axis represents the outcomes of k-fold cross-validation, where the learned $(t, i)$ is applied to other patterns to determine their precision and recall values.
% The analysis reveals that $t = 1.2$ consistently yields higher precision and recall performance, indicating that LLM with higher randomness is better suited for test case generation. 
% Meanwhile, the number of iterations varies among the values between $3$, and $10$, with higher values leading to better results. 
% We also observed that the higher iterations than the choosen $i$ value, always yield same or better precision or recall. 
% However, considering that more iterations can negatively impact efficiency, we decide to choose the least value for $i = 10$, which leads to better precision and recall for \cpats. 
% This combination of $(t, i)$ ensures a good balance between precision, recall, and efficiency for test case generation.


% After selecting a specific $(t, i)$ combination for $V^p$ that effectively generates test cases to classify the variants, we perform 10-fold cross-validation to assess whether this chosen combination can be generalized to other CPATs.
% Let $V^p$ a set of variations generated for a CPAT, where $p \in {1, 2, 3, \ldots, 10}$. After obtaining the optimal combination $(t, i)$ for $V^p$, we then apply this learned combination to all the other $V^{p'}$, where $p' \in {1, 2, 3, \ldots, 10}$ and $p' \neq p$. In other words, we use the same $(t, i)$ values to generate test cases for each $V^{p'}$ in the dataset, allowing us to assess how well this combination generalizes to different patterns represented by different values of $p$. By performing this process for all datasets $V^{p'}$ with $p' \neq p$, we can gain insights into the effectiveness and robustness of the selected combination across the entire dataset, considering all variations represented by different values of $p$.






\begin{figure}[t]
    \begin{minipage}[b]{0.64\linewidth}
        \centering
        \subfigure{
            \includegraphics[width=0.45\linewidth]{images/cross-validation/cross-validation precision.pdf}
        }
        \subfigure{
            \includegraphics[width=0.45\linewidth]{images/cross-validation/cross-validation recall.pdf}
        }
        \vspace{-6mm}
        \caption{Cross-validation results for evaluating optimal $i$ and $t$ values \\ to generate test cases\label{fig:metrics}}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.35\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth,keepaspectratio]{images/temperature_hallucination/temp-0.pdf}
         \vspace{-5mm}
        \caption{Generation of hallucinations along with fixed point iterations ($I_f$)}
        \label{fig:hillusinations}
    \end{minipage}
    \vspace{-10mm}
\end{figure}








% Let $V^p$ be one of the datasets for $p \in {1, 2, 3, \ldots, 10}$, and let $(t, i)$ be the optimal combination obtained for $V^p$. We then apply this learned combination $(t, i)$ to all the other datasets $V^p$, where $p \in {1, 2, 3, \ldots, 10} \setminus {p}$. In other words, we use the same $(t, i)$ values to generate test cases for each $V^p$, allowing us to assess how well this combination generalizes to different patterns in the dataset. 



% Using this updated approach, for each fixed value of $i$, we find the optimal value of $t$ that maximizes the objective function $F(t, i)$, considering precision and recall values for all $t$ in the set $T$. We then check if the improvement in the objective function value achieved by increasing $i$ is significant, and only increase $i$ if the improvement is greater than or equal to the threshold $\delta$. This way, we explore different $t$ values for each fixed $i$ to find the best combination of $t$ and $i$ that maximizes the objective function while keeping the number of iterations low.











% 1. Start with initial values of $t \in T$ and $i \in I$.
% 2. For the fixed value of $i$, compute precision $P(t, i)$ and recall $R(t, i)$ for all $t$ values in the set $T$.
% 3. Calculate the objective function value $F(t, i) = \alpha \cdot P(t, i) + \beta \cdot R(t, i)$ for each computed precision and recall pair.
% 4. Determine the maximum value of the objective function, i.e., $\max_{t \in T} F(t, i)$, and the corresponding value of $t$, denoted as $t_{\text{max}}$, that achieves this maximum.
% 5. If the improvement in the objective function value compared to the previous iteration is greater than or equal to the threshold $\delta$ (i.e., $G(t_{\text{max}}, i) \geq \delta$), update the value of $i$ (e.g., $i = i + 1$) and set $t$ to the value $t_{\text{max}}$.
% 6. Repeat steps 2 to 5 until the improvement in $F(t_{\text{max}}, i)$ falls below the threshold $\delta$ or until $i$ reaches the maximum value in $I$.

% Using this updated approach, for each fixed value of $i$, we find the optimal value of $t$ that maximizes the objective function $F(t, i)$, considering precision and recall values for all $t$ in the set $T$. We then check if the improvement in the objective function value achieved by increasing $i$ is significant, and only increase $i$ if the improvement is greater than or equal to the threshold $\delta$. This way, we ensure that we explore different $t$ values for each fixed $i$ to find the best combination of $t$ and $i$ that maximizes the objective function while keeping the number of iterations low.










% To select optimal (i,t), we define the objective function: $F(t, i) = \alpha \cdot P(t, i) + \beta \cdot R(t, i)$, where $\alpha$ and $\beta$ are weight parameters as before.
% We consider $\alpha > \beta$ as precision of classifying correct variants is more important than recall. 
% Then, we start with initial values of $t \in T$ and $i \in I$.
% Compute the precision $P(t, i)$ and recall $R(t, i)$ for the current values of $t$ and $i$.
% Calculate the objective function value $F(t, i) = \alpha \cdot P(t, i) + \beta \cdot R(t, i)$.
% If the improvement in $F(t, i)$ compared to the previous iteration is greater than or equal to the threshold $\delta$, increase the value of $i$ (e.g., $i = i + 1$).
% Repeat steps 2 to 4 until the improvement in $F(t, i)$ falls below the threshold $\delta$ or until $i$ reaches the maximum value in $I$.
% Using this approach, $i$ will be increased only when there is a significant improvement in the objective function $F(t, i)$, which combines both precision and recall. The optimization process will stop when no further significant improvement can be achieved or when the maximum iteration value is reached.
































% To select optimum $t$ and $i$ combinations, we define our optimization equation as below. 

% \[ O = \frac{2 \cdot (\text{$\frac{1}{|\text{n}|} \sum_{p=1}^{n} \text{$P^p$}(t,i)$}) \cdot  \frac{1}{|\text{n}|} \text{($\sum_{p=1}^{n} \text{$R^p$}(t,i)$}))}{ \frac{1}{|\text{n}|} \text{($\sum_{p=1}^{n} \text{$P^p$}(t,i)$)} + \frac{1}{|\text{n}|} \text{($\sum_{p=1}^{n} \text{$R^p$}(t,i)$)}} - w \cdot i
% \]


% In summary, we employed LLMs to generate test cases for each CPAT. 
% After executing the generated test cases on the oracle, we analyzed the precision and recall to evaluate the effectiveness of the test case generation process. This evaluation involved comparing the classifications made with human-generated test cases for each combination of temperature and iterations.
% Additionally, we calculated the average precision and recall across all CPATs, as depicted in Figure \ref{fig:test_heatmap}.


% In summary, we employed LLM to generate test cases for each CPAT. 
% After executing the generated test cases on the oracle, we analyzed the precision and recall to evaluate the effectiveness of the test case generation process by comparing the classifications made with human-generated test cases for each combination of temperature and iterations.
% Additionally, we calculated the average precision and recall  across all Code Change Patterns, as depicted in Figure \ref{fig:test_heatmap}.

% Finally, we computed the average precision and recall for each combination of $t$ and $i$ for all CPATs, represented as \text{$P^n$}(t,i) and \text{R(t,i)}, respectively. 
% Formally, $\text{$P$}(t,i) = \frac{1}{|\text{n}|} \sum_{p=1}^{10} \text{$P^p$}(t,i),$
% $\text{$R$}(t,i) = \frac{1}{|\text{n}|} \sum_{p=1}^{10} \text{$R^p$}(t,i)$.
% Here, $n$ represents the total number of PATS, which is 10 in this case.





















\resultbox{Higher temperature and more prompt iterations contribute to healthier test cases, resulting in improved precision (\testcaseAvePrecision) and recall (\testcaseAveRecall) for classifying correct and incorrect variants.}





% \input{images/table-evaluations}


\subsubsection{\textbf{What are the optimal parameters for generating unseen variants? :}\label{sec:genvariants}}We employ prompt iteration ($I_p$), and fixed point iteration ($I_f$), to generate a maximum number of variants.
We study the variant generation with respect to iterations and then we fine-tune $I_p$ and $I_f$ by analyzing the variant output for different iteration values.


% While our technique utilizes static analysis and test cases to identify correct variants and static analysis exclusively for selecting applicable variations from the useful ones, we also fine-tune the LLM to reduce the generation of non-useful (i.e., hallucinations) variants and enhance the yield of useful variations. 
% This section provides insights into our fine-tuning methodology for achieving this goal.
% Our objective is to determine the optimal temperature value that maximizes the generation of useful cases and minimizes hallucinations, all while minimizing the iterations, specifically the prompt iteration ($I_p$) and fixed point iterations ($I_f$).


\noindent
\textbf{(A) Prompt iteration $(I_p)$}:
% We repeatedly input the same prompt used to generate variations for a given \cpat in order to generate a larger number of variations. 
We study the number of prompt iterations required for each temperature value until it no longer produces a significant number of new variants, which guides our decision-making regarding the suitable number of prompt iterations for subsequent steps.

\noindent
\textbf{Dataset and Experimental setup:}
We input the CPATs from \Cref{table:cpat} into the LLM alongside a prompt for variant generation, iterating with the same prompts labeled as $i^x_p$ from the 1st to the 100th iteration, where $x$ represents the iteration number.
% This process generates a range of variants. 
Then, we study the cumulative count of distinct variants produced during each iteration.

\noindent
\textbf{Results:} 
\Cref{fig:promptIteration} shows the process of variant generation for the initial 10 iterations at temperature 0.
In the first iteration, the LLM generated an average of 70\% (with a minimum of 45\% and a maximum of 82\%) of total variants. 
By the second iteration, this increased to 83\% (with a minimum of 68\% and a maximum of 96\%) of variants. 
During the third iteration, the LLM generated 95\% (with a minimum of 85\% and a maximum of 100\%) of variants. 
Beyond that point, we observed that the LLM hardly generates any new variants for a given \cpat. 
Hence, we decided to perform prompt iterations three times to generate variants for a given \cpat.
This observation is consistent across all temperature values, and we have included the analysis plots on the companion website~\cite{artifacts}.

% right temperature value that we need to consider in order to get the variations with fewer iterations.  

% \begin{figure}[htbp]
%     \includegraphics[width=0.49\textwidth,keepaspectratio]{images/prompt_iteration/line_plot.pdf}

%     \caption{}
%     \label{fig:promptIteration}

% \end{figure}



\resultbox{Continuing prompt iterations indefinitely is an option to generate numerous variants. However, beyond the third iteration, LLM produces new variants sparingly.}


\noindent
\textbf{(B) Fixed-point iteration $(I_f)$:}
In order to generate as many variants as possible, we perform Fixed-point iteration by inputting a applicable variant generated in the previous step to the LLM. 
While this approach can potentially generate many of variants, it can also lead to producing numerous hallucinations (not-useful) when the LLM is prompted with another hallucination. This situation can impact the performance of \tool in two ways: 
\begin{enumerate*}[label=(\roman*)]
\item multiple iterations generating hallucinations, 
and 
\item inferring rules for hallucinations that will not be applied to the code.
\end{enumerate*}
We study the generation of useful variants along with the number of fixed-point iterations.

%\noindent
\textbf{Dataset and Experimental setup:} 
We use the oracle mentioned in \Cref{sec:oracal} to study this in two ways. 
\begin{enumerate*}[label=(\roman*)]
\item We study, for each temperature, the cumulative ratio of non-useful variants to total non-useful variants in the oracle, generated at each fixed-point iteration.
This analysis helps us understand how hallucination generation trends with increasing fixed-point iterations.
% allowing us to identify the suitable number of iterations to prevent excessive hallucinations.
% The analysis results are shown in \Cref{fig:hillusinations},
\item In addition to minimizing hallucinations, it is also important to increase the number of useful cases. 
Hence, we study the generation of useful cases in along with iterations and temperature.
\end{enumerate*}




% \noindent
\textbf{Results:} 
The plot in \Cref{fig:hillusinations} shows the distribution of the ratio of the cumulative number of hallucinations generated by each iteration relative to the total hallucinations in the oracle.
This analysis is conducted for each \cpat listed in \Cref{table:cpat}, represented by lines in each plot, and across various temperature values.
While \Cref{fig:hillusinations} presents the plot for only temperature 0, the others showcase similar trends as depicted in the provided plots and are available on our companion website~\cite{artifacts}.
We noticed a consistent trend across all temperatures and each \cpat, where the generation of hallucinations begins after approximately 3 to 6 fixed-point iterations, followed by a rapid increase.
While the graphs suggest that reducing hallucinations is more achievable with fewer fixed-point iterations, a trade-off arises because we also aim to increase the generation of useful variants. 
To address this, we analyzed the cumulative ratio of useful variants generated up to each iteration compared to the total variants generated, across different temperature values.
Consistently across all \cpats, we observed that temperatures within the middle range, i.e, 0.5 and 0.7, consistently yield useful variants with fewer fixed-point iterations compared to other temperatures.
For example, with four fixed-point iterations, temperatures 0.5 and 0.7 yield useful variants spanning 61\% to 83\% for each \cpat; this percentage rises to 69\% to 88\% with five iterations, and the trend persists with further iterations.  
% However, it is important to note that increasing fixed-point iterations also increases the occurrence of hallucinations.
Considering the goal of generating variations while maximizing useful variants and minimizing hallucinations, we determined that performing five fixed-point iterations and focusing on variations generated at the middle temperatures 0.5 and 0.7 is an optimal approach.
Using these settings, we further apply \tool in \Cref{sec:rq4} and \Cref{sec:rq6} to compare its effectiveness against the baseline, followed by presenting the generated variants to actual developers for usefulness evaluation.









% \begin{figure}[]
% \subfigure{
% \includegraphics[width =0.3\textwidth]{images/temperature_hallucination/temp-0.pdf}}
% \subfigure{
% \includegraphics[width =0.3\textwidth]{images/temperature_hallucination/temp-0.3.pdf}}
% \subfigure{
% \includegraphics[width =0.3\textwidth]{images/temperature_hallucination/temp-0.5.pdf}}
% \vspace{-3.5ex}

% % \subfigure{
% % \includegraphics[width =0.3\textwidth]{images/temperature_hallucination/temp-0.7.pdf}}
% % \subfigure{
% % \includegraphics[width =0.3\textwidth]{images/temperature_hallucination/temp-0.9.pdf}}
% % \subfigure{
% % \includegraphics[width =0.3\textwidth]{images/temperature_hallucination/temp-1.2.pdf}}
% % \vspace{-4ex}
% \caption{Generation of hallucinations for each temperature and iteration ($I_f$):
% Y-axis is the ratio of the cumulative number of hallucinations generated by each iteration (given in X-axis) to the total hallucinations in the oracle\label{fig:hillusinations}}
% \vspace{-4mm}
% \end{figure}




% \subsubsection{\textbf{Maximizing useful variations:}}


\resultbox{Medium temperatures yield fewer hallucinations and more useful variants, all while requiring fewer fixed-point iterations.}


